Can ChatGPT pass the Vietnamese National High School Graduation Examination?

This research article highlights the potential of AI-powered chatbots in education and presents the results of using ChatGPT, a large language model, to complete the Vietnamese National High School Graduation Examination (VNHSGE). The study dataset included 30 essays in the literature test case and 1,700 multiple-choice questions designed for other subjects. The results showed that ChatGPT was able to pass the examination with an average score of 6-7, demonstrating the technology's potential to revolutionize the educational landscape. The analysis of ChatGPT performance revealed its proficiency in a range of subjects, including mathematics, English, physics, chemistry, biology, history, geography, civic education, and literature, which suggests its potential to provide effective support for learners. However, further research is needed to assess ChatGPT performance on more complex exam questions and its potential to support learners in different contexts. As technology continues to evolve and improve, we can expect to see the use of AI tools like ChatGPT become increasingly common in educational settings, ultimately enhancing the educational experience for both students and educators.

==> score.tex <==
 7.6, 8.6, 7.6, 8, 7.8
 6, 7, 6.25, 8.25, 7.75
 7.5, 6.89, 7.5, 5.63, 6.48
 5, 5.25, 7.5, 6.25, 6.75
 6, 6.25, 6, 6.5, 5.75
 5.2, 6.6, 6, 6.2, 5.4
 6, 6, 5.25, 5.75, 6
 4.25, 4.75, 5.5, 6, 7.75
 4, 4.25, 6.25, 4.75, 4.75

